Prompt and non-prompt $J/\psi$ elliptic flow in Pb+Pb collisions at $\sqrt{s_{_\text{NN}}} = 5.02$ TeV with the ATLAS detector

The elliptic flow of prompt and non-prompt $J/\psi$ was measured in the dimuon decay channel in Pb+Pb collisions at $\sqrt{s_{_\text{NN}}}=5.02$ TeV with an integrated luminosity of $0.42~\mathrm{nb}^{-1}$ with the ATLAS detector at the LHC. The prompt and non-prompt signals are separated using a two-dimensional simultaneous fit of the invariant mass and pseudo-proper decay time of the dimuon system from the $J/\psi$ decay. The measurement is performed in the kinematic range of dimuon transverse momentum and rapidity $9<p_\mathrm{T}<30$ GeV, $|y|<2$, and 0-60% collision centrality. The elliptic flow coefficient, $v_2$, is evaluated relative to the event plane and the results are presented as a function of transverse momentum, rapidity and centrality. It is found that prompt and non-prompt $J/\psi$ mesons have non-zero elliptic flow. Prompt $J/\psi$ $v_2$ decreases as a function of $p_\mathrm{T}$, while non-prompt $J/\psi$ it is, with limited statistical significance, consistent with a flat behaviour over the studied kinematic region. There is no observed dependence on rapidity or centrality.

==> HION-2017-05-PAPER-auxmat.tex <==
\part*{Auxiliary material}
\addcontentsline{toc}{part}{Auxiliary material}
%-------------------------------------------------------------------------------
\begin{figure}[h!]
\begin{center}
	\includegraphics[width=8cm]{fit_uncert_mass_pull_pt_1_1}
	\includegraphics[width=8cm]{fit_uncert_time_pull_pt_1_1}
%	\includegraphics[width=8cm]{fit_mass_pt_1_1}
%	\includegraphics[width=8cm]{fit_time_pt_1_1}
\caption{Fit projections of the two-dimensional invariant mass ($m_{\mu\mu}$) and pseudo-proper decay time ($\tau_{\mu\mu}$) for the signal extraction for the first azimuthal bin $0 < 2|\phi-\Psi_2| < \pi/4$ in the kinematic range $9 < \pT < 11~\GeV$, $0<|y|<2$ and 0 - 60\% centrality. The pulls are plotted together with the systematic uncertainties associated to variations of the probability density function defined for the signal extraction.}
\end{center}
\end{figure}
%-------------------------------------------------------------------------------
\begin{figure}[h!]
\begin{center}
	\includegraphics[width=8cm]{Figure_Pt_Prompt_and_Nonprompt}
\caption{Comparison of prompt (blue) and non-prompt (red) \jpsi $v_2$  as a function of transverse momentum for the rapidity interval $|y| < 2$ and centrality $0-60\%$. The statistical and systematic uncertainties are shown using vertical error bars and boxes respectively. The horizontal error bars represent the kinematic range of the measurement for each bin.}
\end{center}
\end{figure}
%-------------------------------------------------------------------------------
\begin{figure}[h!]
\begin{center}
	\includegraphics[width=8cm]{Figure_Rap_Prompt_and_Nonprompt}
\caption{Comparison of prompt (blue) and non-prompt (red) \jpsi $v_2$ as a function of rapidity for transverse momentum in the range $9 < \pT < 30~\GeV$ and centrality $0-60\%$. The statistical and systematic uncertainties are shown using vertical error bars and boxes respectively. The horizontal error bars represent the kinematic range of the measurement for each bin.}
\end{center}
\end{figure}
%-------------------------------------------------------------------------------
\begin{figure}[h!]
\begin{center}
	\includegraphics[width=8cm]{Figure_Npart_Prompt_and_Nonprompt}
\caption{Comparison of prompt (blue) and non-prompt (red) \jpsi $v_2$ as a function of average number of nucleons participating in the collision for transverse momentum in the range $9 < \pT < 30~\GeV$ and rapidity $|y| < 2$. The statistical and systematic uncertainties are shown using vertical error bars and boxes respectively. The centrality interval associated to a given value of \avgNpart is written below each data point.}
\end{center}
\end{figure}
%-------------------------------------------------------------------------------
\begin{table}[t!]
\centering
%\begin{tabular}{@{} ccc @{}} % Column formatting, @{} suppresses leading/trailing space
\begin{tabular}{cccc}
\toprule
Centrality  & \avgNpart 		& $N_{\mu\mu}^{\text{raw}}$ & $\mathcal{R}$\\
\midrule
$0-20\%$    & $311.4 \pm 2.6$  	& 17114 & $0.759\pm0.011$ \\
$20-40\%$   & $160.3 \pm 2.7$  	& 8942 & $0.871\pm0.004$ \\
$40-60\%$   & $70.5 \pm 2.2$  	& 3372 & $0.766\pm0.006$ \\
$0-60\%$    & $135.6 \pm 2.0$  	& 29428 & $0.794\pm0.032$ \\
\bottomrule
\end{tabular}
\caption{The average number of participating nucleons, \avgNpart, the number of raw dimuon candidates per centrality class, $N_{\mu\mu}^{\text{raw}}$, in the invariant mass range $2.6 < m_{\mu\mu} < 3.5$ \GeV, and the event-plane resolution, $\mathcal{R}$, values with their total uncertainties in each centrality interval.}
\end{table}

==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
PDFLATEX = pdflatex
BIBTEX   = biber

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Change biblatex backend
bibtex: $(BASENAME).tex
	if [ $(BIBTEX) = 'biber' -o $(BIBTEX) = 'bibtex' ]; then \
	  echo "Changing biblatex backend in $<"; \
	  sed -i'.bak' -e 's/backend=biber/backend=$(BIBTEX)/' -e 's/backend=bibtex/backend=$(BIBTEX)/' $<; \
	else echo "Invalid value for BIBTEX: $(BIBTEX)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf

